Optimized Look-Ahead Tree Policies: A Bridge Between Look-Ahead Tree Policies and Direct Policy Search

Direct policy search (DPS) and look-ahead tree (LT) policies are two widely used classes of techniques to produce high performance policies for sequential decision-making problems. To make DPS approaches work well, one crucial issue is to select an appropriate space of parameterized policies with respect to the targeted problem. A fundamental issue in LT approaches is that, to take good decisions, such policies must develop very large look-ahead trees which may require excessive online computational resources. In this paper, we propose a new hybrid policy learning scheme that lies at the intersection of DPS and LT, in which the policy is an algorithm that develops a small look-ahead tree in a directed way, guided by a node scoring function that is learned through DPS. The LT-based representation is shown to be a versatile way of representing policies in a DPS scheme, while at the same time, DPS enables to significantly reduce the size of the look-ahead trees that are required to take high-quality decisions. We experimentally compare our method with two other state-of-the-art DPS techniques and four common LT policies on four benchmark domains and show that it combines the advantages of the two techniques from which it originates. In particular, we show that our method: (1) produces overall better performing policies than both pure DPS and pure LT policies, (2) requires a substantially smaller number of policy evaluations than other DPS techniques, (3) is easy to tune and (4) results in policies that are quite robust with respect to perturbations of the initial conditions.

==> conclusion.tex <==
This paper has introduced \textit{optimized look-ahead tree policies, a novel technique} that bridges the gap between two major families of solutions for solving sequential decision-making problems: direct policy search (DPS) and look-ahead tree (LT) policies. 
Our approach uses a new way of representing a policy by using parameterized look-ahead trees. In this representation, the parameters of the policy over which optimization takes place encode the node scoring function by which the tree is grown (until a predefined computational budget is exhausted) every time an action is required from the system. This approach manages to combine the best of both DPS and LT approaches. From the point of view of DPS, optimized look-ahead tree policies provide a highly-generic way of representing policies that alleviates the need to choose a complex function approximator. From the point of view of LT, DPS is the key that enables to significantly reduce the online computational requirement, through a principled  offline parameter-learning procedure.

We have shown through an extensive experimental study that our approach has several qualities: it (1) produces high-performance policies that often outperform both pure LT policies and pure DPS policies, (2)  requires at the offline training stage a substantially smaller number of policy evaluations than other DPS techniques, thanks to a small parameter space whose size does not depend on the policy complexity, (3) is easy to tune since it avoids having to choose a particular function approximator and (4) results in policies that are quite robust with respect to perturbations of the initial states.
Compared to traditional LT policies, we have shown that learning a node scoring function can result in substantial savings in terms of required online computational resources.

This paper has focused on a particular kind of sequential decision-making problems:  finite actions, deterministic transitions, known transition and reward 
function (i.e., a generative black-box model which allows us to simulate arbitrary transitions), and an ``informative'' reward. However, we believe that except for the last item, all the other items on this list can be addressed in future work. 
For example, large number of actions means that we can no longer exhaustively generate all successor 
states when predicting one step ahead; instead, one would have to use sampling techniques or progressive widening
techniques which is also an active research topic in tree-based search \cite{a1,a2,a3,a4}. Deterministic transitions can be relaxed to 
weakly stochastic transitions (weakly meaning that there is only a small number of possible successor
states) as was done in \cite{busoniu_adprl11} to extend the optimistic strategy from \cite{Hren08} to
sparse stochastic systems. And finally, in application scenarios where a generative model is not 
available from the beginning, one could also try to integrate model-learning over time into the 
policy search framework (e.g., see \cite{jung_ecml10}).  


==> introduction.tex <==

% Introduire les deux familles
A wide range of techniques have been developed in the last decades for solving optimal sequential decision-making problems in the fields of optimal control and reinforcement learning. Two important classes of techniques that are known to work well on difficult problems characterized by large state spaces are \textit{direct policy search} (DPS) \cite{bibO} and \textit{look-ahead tree} (LT) policies \cite{Hren08}. 

% DPS
In DPS, a policy is seen as a parameterized function that maps states to actions. In order to identify the best settings of the parameters, DPS techniques rely on local or global optimization algorithms that directly maximize the performance of the policy estimated through simulation or real-world experiments. DPS avoids learning value functions and all the complexities involved with approximating them. Instead, optimization is carried out directly in policy space. The rationale for doing this is that, while usually the value function will be a rather complex object and thus thought to be hard to approximate, a control policy will often be a much ``simpler'' object and thus could also be (so it is believed) much easier to learn. Note that in DPS approaches, making a decision is generally a very fast operation while all heavy computations are performed in an offline way, when optimizing the parameters of the policy.

% LT
Look-ahead tree policies rely on a totally different principle than DPS, since they have no parameters that need to be learned in an offline way: all the computational work is done online during each decision-making step. In order to take each single decision, a LT policy proceeds in two steps: first, it develops a look-ahead tree by simulating the evolution of the system subject to multiple possible future action sequences, then, it selects an action based on the information collected in this tree. The quality of decisions taken by LT policies depends on the size of the tree: the more action sequences have been tried, the better the final decision will be. The computational complexity of an LT policy can thus be adjusted by changing the size of the look-ahead tree, small trees leading to fast approximate decisions and large trees leading to expensive high-quality decisions.

% Avantage et inconvenients
Both DPS and LT techniques have their strengths and weaknesses.
%
DPS can often produce, with comparatively little effort, good policies for difficult control problems where typical value function based methods would otherwise fail. However, a major issue in DPS is that the final performance strongly depends on the choice of an appropriate policy representation. Common policy representations include linear parametrizations \cite{heidrich-meisner08}, neural networks \cite{moriarty99,stanley_neat02,gomez08} or radial basis functions \cite{bibF,deisenroth_pilco11} and typically have hyper-parameters that require tuning (e.g. the number of hidden neurons). For a given problem, choosing an appropriate representation and tuning its hyper-parameters is a difficult problem, which typically involves a large amount of trial and error. 
%
On the other hand, this effort is not required with LT policies thanks to the look-ahead tree that acts as a unified built-in highly generic representation of the decision problem. Hence, LT policies can be applied to almost any sequential decision-making problem without any prior knowledge -- this without even depending on the dimensionality of the state space. The main issue with LT policies is that they typically require a large amount of online computational resources to produce high-quality decisions. In practice, these resources are often limited, either due to real-time constraints (e.g. $100$ ms per decision) or human-scale constraints (e.g. one hour or one day per decision). Given such a constraint and given the difficulty of the problem, the actions suggested by LT policies may be arbitrarily sub-optimal. 

% Combinaison
LT policies alleviates the need to choose a complex approximation structure for policies, while at the same time DPS offers a principled way of reducing online computational requirements through an offline learning procedure. Starting from two these observations, it is natural to wonder how we can combine these two ideas in order to create a new hybrid solution for sequential decision-making that leverages the advantages of both.

% Contribution + L'introduire en partant de LT
In this paper, we propose to bridge the gap between LT and DPS policies with a new hybrid technique: \textit{optimized look-ahead tree (OLT) policies}\footnote{This technique was initially proposed in \cite{bibA} and is here extended through a more mature exposition of the method and an extensive experimental study which covers much more aspects than the initial paper. Furthermore, we introduce the use of Gaussian process optimization to improve the sample efficiency of the approach.}. From the point of view of LT policies, our approach starts from the observation that the efficiency of an LT policy, given a finite computational budget, can be improved by directing the way in which the tree is grown, for example by giving priority to sequences of actions that seem more promising \cite{Hren08}. In fact, a large number of different strategies could be considered to develop look-ahead trees, by combining aspects from breadth-first exploration to depth-first exploration and from random exploration to purely greedy exploration. In practice, the quality of these different strategies depend on the characteristics of the problem (e.g. to which extent are rewards informative about the long-term goal?), on the available online computational budget, and may even also depend on the current location in the state-space. Optimized look-ahead trees then consist in parameterizing a node scoring function that encodes the way in which look-ahead trees are grown and then learning the best values of these parameters in a problem-driven way through DPS. 

% Discussion du cote DPS
%Note that, from the point of view of DPS, our approach is quite unusual. 
Traditionally, policies in DPS rely on an approximation structure, which is usually one of those used in supervised learning. These approximation structures lead to policies which are representable through simple mathematical formulas, such as the maximization of a linear dot-product or the computation of a feed-forward neural network. Note however that, choosing such a policy or an OLT policy does not make any conceptual difference for DPS: as any other policy, OLT policies may be viewed as functions that receive a state, perform some parameter-dependent internal computations and then return an action. The distinguishing feature of OLT policies is that their internal computations rely on explicitly exploiting a generative model of the problem.

% Resultats
We experimentally compare our hybrid method with two other state-of-the-art DPS techniques, where the policies are represented through neural networks and adaptive radial basis functions, respectively. We also consider LT policies with four different exploration strategies. Based on an extensive study on four challenging benchmark domains, we show that our approach indeed leverages the advantages of the two techniques from which it originates. In particular, we show first that OLT policies perform often significantly better than both pure DPS and pure LT policies and that they are at least competitive in all cases. Second, thanks to their use of a model, it turns out that OLT policies require a substantially smaller  number of parameters than neural networks and radial basis functions to reach high-performance policies. In turn, they require, as shown in the experimental results, significantly less offline policy
evaluations than other DPS techniques. Third, %since our technique avoids the need to choose and tune a particular approximation structure, 
we show that OLT policies are much more straightforward to train as compared to usual DPS which often requires cumbersome trial and error iterations to choose and train their approximation structure. Finally, we show that OLT policies are quite robust with respect to perturbations of the initial conditions.  

% Plan
The content of the paper is structured as follows. In Section~\ref{sec:problem}, we begin by introducing basic notation and state formally the type of sequential decision-making problems this paper is about. Section~\ref{sec:contribution} presents a detailed description of optimized look-ahead trees. The node scoring function of optimized look-ahead trees can be learned using any derivative-free global optimizer. One such optimizer which was shown to be highly relevant to DPS is Gaussian process optimization \cite{frean_gpo08,lizotte07}. We give a brief (but for all practical purposes fully sufficient) summary  of this approach in Section~\ref{sec:gpo}. 
%
Section~\ref{sec:experiments} presents the results of  extensive experimental 
evaluations, wherein we compare optimized look-ahead trees with different pure DPS and pure LT techniques on a number of well-known benchmark domains. We present related work in Section~\ref{sec:related work} and finally conclude in Section~\ref{sec:conclusions}.



==> related.tex <==
The approach proposed in this paper lies at the intersection of two families of solutions for sequential-decision making. We first overview \textit{direct policy search} in Section \ref{ssec:dps} and then discuss relevant work on \textit{look-ahead tree search} in Section \ref{ssec:lt}. Section \ref{ssec:mpc} positions our approach with respect to Model
Predictive Control techniques. Finally, Section \ref{ssec:parameterizedalgo} suggests that optimized look-ahead tree policies belong to a larger emergent class of techniques: \textit{parameterized algorithms for decision-making}.

\subsection{Direct policy search}
\label{ssec:dps}


% DPS: gradient free / gradient-based
Direct policy search is a widely used class of solutions that comes from reinforcement learning. For a general overview over the field of reinforcement learning, refer to one of the books of \cite{sutton98introduction,bert07dpvolii,powell07,bibO}. Over the years, many DPS techniques have been proposed and giving credit to every one of them would be hardly possible. Individual techniques differentiate  themselves by their policy parametrization and the optimization method used for identifying parameters leading to a high-performing policy. The main distinction is whether the 
policy search is \textit{gradient-free} or \textit{gradient-based}.

% Gradient-based DPS
Gradient-based DPS, which very often also goes by the name of policy-gradient
method, follows an iterative optimization scheme and uses the gradient of the value
function to adapt and change the policy parameters such that performance increases. 
This requires the value function to be a smooth function of the policy parameters, which
is typically achieved by considering compatible stochastic policies. Often however, 
the gradient cannot be computed analytically since the value function itself
is not available in closed form. Instead, the gradient has to be estimated using, e.g., 
finite difference approximation, Monte-Carlo rollouts or value function approximation
which leads to the actor-critic methods. One of the best known examples is probably 
the natural policy gradient method described in 
\cite{peters_naturalactorcritic07}; another more recent example is the work in 
\cite{deisenroth_pilco11}. While impressive results have been obtained in particular
for learning controllers in robotics, policy-gradient methods do have some weaknesses;
the most notable ones being a high sensitivity to the initial value of the policy
parameters (the starting point of the iteration), abundance of local minima, and
difficulties when the return is noisy or stochastic. Note that in this paper we do not
deal with gradient-based policy search.

% Gradient-free DPS
Gradient-free DPS on the other hand finds the best policy parameters via derivative-free
global optimization. Its main strength is simplicity and generality; the latter meaning that,
because it is derivative-free, the representation of a policy by any algorithm with adjustable
parameters is admissable, and not only those for which the value function will be differentiable.
Since gradient-free DPS techniques perform a global search in the parameters space, they do not suffer from local minima or from the problem of having to guess a good initial solution; these techniques were also shown to cope well with
stochastic returns and hidden states. For certain domains in reinforcement learning such as Tetris,
the best performing policies known today have been obtained by gradient-free DPS (see \cite{szita06} and follow-up work). The weakness of this approach is that conceptually it is less sample-efficient than policy-gradient methods and thus will require a substantially higher
number of policy evaluations. This comes as a consequence of having to solve a global optimization problem over a potentially high-dimensional search space; however, by carefully designing the policy parametrization and choosing powerful optimizers sample efficiency is often improved.

% First work in Gradient-free DPS
Early examples of DPS came under the guise of evolutionary approaches to reinforcement learning, or neuroevolution, and consisted of neural networks as policy representation, with the weights making up the policy parameters, and variants of genetic algorithms acting as global optimizer. Examples can be found in \cite{moriarty99} and \cite{gomez03}, where later work also considered optimization of the network structure
\cite{stanley_neat02}, or using recurrent neural networks to better cope with hidden states \cite{gomez08}. A recent comparison of these methods can also be found in  \cite{whiteson10} and \cite{shivaram11}.

% More recent work
As an alternative to genetic algorithms, more recent work started to explore the use of the
cross-entropy method \cite{crossentropy}, or variants such as the covariance matrix
adaptation evolution strategy CMA-ES \cite{cma-es} as global optimizer for policy
search. Examples include \cite{heidrich-meisner08}, where the policy was represented by 
a simple linearly parametrized function, \cite{shivaram11}, where the policy was 
represented by a neural network, or \cite{bibF}, where the policy was represented by 
adaptive radial basis functions. These latter two were also used in this paper as baseline
methods during the experimental evaluation of our look-ahead trees. Another example for a 
policy parametrization is to use domain-specific building blocks, such as motor primitives,
as it was done in \cite{kohl04} and \cite{lizotte07} to optimize the gait of the AIBO
quadrupedal robot. A different kind of policy representation is used in \cite{szita07}
to learn a policy for the game of Ms. Pac-Man; here the policy is represented by a list
of domain-specific parameterized rules.

% GPO
Section \ref{sec:gpo} described a third option for the global optimization part: Gaussian process optimization \cite{mockus89bayesianoptim,DBLP:journals/corr/abs-1012-2599}. GPO can achieve very good sample efficiency and was previously considered for policy search in \cite{lizotte07} and \cite{frean_gpo08}. In the end however, the choice of which global optimizer one uses will always be secondary; what is more important is how the policy is represented and to what extent this representation facilitates the optimization process by shaping the  ``fitness landscape''.   
 
\subsection{Look-ahead tree search}
\label{ssec:lt}

% Planning and search
The algorithm studied in this paper can also be related to the larger field of tree-based planning and search. One of the most seminal works in this  field is the $A^*$ algorithm \cite{bibH} which uses a best-first search to find the shortest path from a source state/configuration to a goal state/configuration. The conceptual difference between $A^*$ and related methods on the one side and what we are presenting here on the 
other side is that our method implements an {\em online} and {\em finite computational budget} mechanism: a search tree is grown at each decision-making step, and only a finite number of node expansions are allowed during tree development  (the larger the computational budget, the better the decision). In $A^*$ the search tree needs to be grown until a goal state is reached. Our method is thus capable of online planning and producing closed-loop policies, whereas $A^*$ is not. 
%
More specifically, the algorithm studied in this paper can also be interpreted as a method for {\em learning} an exploration strategy in a tree. In $A^*$, the function used for evaluating the nodes is the sum of two terms: the length of the 
so far shortest path from the source to the current node and an optimistic estimate 
of the shortest path from this node to the goal (a so-called ``admissible'' heuristic). 
Several authors have sought to learn good admissible heuristics for the $A^*$ algorithm. 
For example, we can mention the LRTA$^*$ algorithm \cite{bibI} which is a variant of A$^*$
and which learns over multiple trials an optimal admissible heuristic. More recent work for
learning strategies to efficiently explore graphs have focused on the use of supervised regression techniques using various approximation structures to solve this problem (e.g., linear regression, neural networks, $k$-nearest neighbors); for example, see \cite{bibJ,bibK,bibL,bibH}. The objective of which node to best explore next also arises in the context of game-playing; here we can mention, e.g., Monte-Carlo tree search \cite{a2}. In particular progressive strategies which widen up the actions (nodes considered for expansion) such as in \cite{a1,a2,a3} and which
can also be used for continuous action spaces \cite{a4} could be a promising enhancement for the policy search technique presented herein.  

\subsection{Model predictive control}
\label{ssec:mpc}

Model Predictive Control techniques have originally been introduced as
ways to stabilize large-scale systems with constraints around
equilibrium points (or around a reference trajectory) \cite{Morari1999MPC,Coen2008MPC,Ernst09RLMPC}. They exploit an explicitly formulated model of the problem and solve in a receding horizon manner
a series of finite time open-loop deterministic optimal control
problems. In such they are very much related to look-ahead tree
techniques. Actually, a MPC technique that searches for the first
action of the optimal sequence of actions over the finite optimisation
horizon through (clever) exploration of a tree is a look-ahead tree
technique. However, most of the control techniques labelled as MPC
techniques do not use tree-exploration for identifying
(near-) optimal sequences of actions. They rather assume strong
regularity assumptions on the system dynamics and the reward function
(e.g., linearity) -- that we do not make here -- which are exploited to
reformulate the search for an optimal open-loop sequence of action as
a standard mathematical programming problem (e.g., convex optimisation
problem, mixed integer programming problem). This reformulation of the
problem as a mathematical programming problem often leads to
techniques that are able to scale well to very large state-action
spaces, provided of course that the regularity assumptions hold.

\subsection{Parameterized algorithms for decision-making}
\label{ssec:parameterizedalgo}

Our work relies on a rather simple and generic research methodology: for a given targeted class of problems, (i) identify an algorithm skeleton that is believed to provide promising solutions to problem instances, (ii) parameterize this algorithm and (iii) optimize the parameters in a problem-driven way, through DPS, i.e., through direct optimization of the algorithm performance. This methodology can be applied to a wide range of problem kinds and has already inspired several authors. The system proposed in \cite{bibG} places  an optimisation layer on top of an approximate value 
iteration algorithm to optimize the location of its basis functions. In \cite{bibN} (Section 5.3), the authors consider multi-stage stochastic
programming techniques and optimize the scenario trees using Monte-Carlo methods. Closer to our work, it is proposed in \cite{couetoux2012ExploUCT} to parameterize a tree-search technique for decision-making: \textit{upper confidence trees}. In this work, the parameters enable to control the simulation policy used to estimate long-term returns within the upper confidence tree algorithm. 

Parameterized algorithms have also been shown to be relevant to solve various kinds of exploration / exploitation dilemma in a problem-driven way. References \cite{Maes2012Icaart} and \cite{Maes11EWRLb} propose to  learn exploration / exploitation strategies
for multi-armed bandit problems either by using the same kind of parameterizations (a simple linear function)
and the same kind of optimizers (derivative-free global optimizers) as ours or by searching in a space of formulas. Reference  \cite{Castronovo2012Ewrl} extends this idea to the exploration / exploitation dilemma that occurs in single-trajectory reinforcement learning. Here, the parameters are no more real-valued vectors, but rather small formulas that depend on the internal variables of the policy. Given a target class of Markov decision problems, this method is able to learn high-performance policies that outperform state-of-the-art generic reinforcement learning algorithms.

We believe that with the recent progress in derivative-free global optimization (with algorithms such as cross-entropy, CMA-ES and GPO) and the continuously growing available computing power, the class of such parameterized algorithms optimized in a problem-driven way has high chances to grow in the near future, since they offer a systematic way to improve upon generic solutions, by exploiting problem-dependent characteristics through learning.


